On the Adaptation to Concept Drift for CTR Prediction

Click-through rate (CTR) prediction is a crucial task in web search, recommender systems, and online advertisement displaying. In practical application, CTR models often serve with high-speed user-generated data streams, whose underlying distribution rapidly changing over time. The concept drift problem inevitably exists in those streaming data, which can lead to performance degradation due to the timeliness issue. To ensure model freshness, incremental learning has been widely adopted in real-world production systems. However, it is hard for the incremental update to achieve the balance of the CTR models between the adaptability to capture the fast-changing trends and generalization ability to retain common knowledge. In this paper, we propose adaptive mixture of experts (AdaMoE), a new framework to alleviate the concept drift problem by statistical weighting policy in the data stream of CTR prediction. The extensive offline experiments on both benchmark and a real-world industrial dataset, as well as an online A/B testing show that our AdaMoE significantly outperforms all incremental learning frameworks considered.

==> admoe_arxiv/exp.tex <==



\section{Experiments}


% In this section, we evaluate the performance of AdaMoE through offline experiments on both industrial dataset and public dataset, as well as an online A/B test. 

% \hl{Due to the absence of the public dataset to study concept drift in CTR Prediction task, we reorganized the Avazu Dataset by timestamp to ensure chronological order. Further experiments have been conducted to verify the effectiveness of the proposed framework on public benchmarks.}


% \subsection{Offline Experiments}

% \textbf{Datasets.} 
\subsection{Datasets and Evaluation Metrics}
\textbf{Industrial Dataset}.
The industrial dataset is extracted from the user logs of one of world's largest E-commerce companies.
The extracted dataset includes about 4.5 billion ad impression records within one day.
The collected data is sorted in chronological order and divided into datasets.
Each dataset $\mathcal{D}_t$ contains 2048 samples.
% This constitutes the data stream for offline experiments.

\textbf{Public Dataset}. Due to the absence of the public dataset to study concept drift in CTR Prediction task, here we adopt the Avazu dataset\footnote{\url{https://www.kaggle.com/c/avazu-ctr-prediction/data}}, which includes the timestamp information of impressed advertisement. There are 40,428,967 records over 10 days.
% from October 21, 2014 to Octorber 30, 2014. 
We use the records of the first 3 days to pretrain models. For the records of the rest 7 days, we sort them in chronological order, and split them into stream dataset $\mathcal{D}_t$ by a fixed interval of an hour due to the timestamp granularity in the Avazu dataset.
In the experiments, the stream dataset $\mathcal{D}_t$ is consumed sequentially. Stream dataset $\mathcal{D}_t$ is first evaluated by the model trained with previous data. Then, $\mathcal{D}_t$ is used to train the model. Our code, including data preprocessing and model implementation, will be publicized on acceptance.

% \begin{table}[t]
%   \caption{The Overall AUC on Avazu over 3-Run, std$\approx10^{-4}$. \#(Exp.) denotes number of experts.}
%   \label{tab:benchmark-res}
%   \centering
% %   \small
% \begin{tabular}{c|cccc}
%    \toprule
%    \#(Exp.) & IncCTR & MoE & IADM & AdaMoE \\
%    \midrule
%     %1 & 0.7603 & 0.7612 & 0.7619 & \textbf{0.7620} \\
%     3 & 0.7594 & 0.7599 & 0.7614 & \textbf{0.7624} \\
%     5 & 0.7591 & 0.7558 & 0.7597 & \textbf{0.7619} \\
%     7 & 0.7589 & 0.7547 & 0.7157 & \textbf{0.7621} \\
%     9 & 0.7590 & 0.7524 & 0.7170 & \textbf{0.7617} \\
%    \bottomrule
% \end{tabular}
% \end{table}
\begin{table}[t]
  \caption{Overall AUC on Industrial and Avazu dataset over 3-Run, std$\approx10^{-4}$. \#(Exp.) denotes number of experts.}
  \label{tab:main-res}
  \centering
  \small
\resizebox{1\columnwidth}{!}{ 
\begin{tabular}{c|c|cccc}
   \toprule
   Dataset & \#(Exp.) & IncCTR & MoE & IADM & AdaMoE \\
   \midrule
   \multirow{4}{*}{Industrial(DCN)} & 3 & 0.7569 & 0.7578 & 0.7582 & \textbf{0.7590} \\
                        & 6 & 0.7571 & 0.7580 & 0.7578 & \textbf{0.7597} \\
                        & 9 & 0.7568 & 0.7579 & 0.7576 & \textbf{0.7593} \\
                        & 12 & 0.7563 & 0.7573 & 0.7571 & \textbf{0.7585} \\
   \midrule
   \multirow{4}{*}{Industrial(DIN)} & 3 & 0.7631 & 0.7635 & 0.7643 & \textbf{0.7663} \\
                        & 6 & 0.7635 & 0.7638 & 0.7642 & \textbf{0.7664} \\
                        & 9 & 0.7633 & 0.7636 & 0.7640 & \textbf{0.7660} \\
                        & 12 & 0.7628 & 0.7631 & 0.7633 & \textbf{0.7657} \\
    \midrule
    \multirow{4}{*}{Avazu} & 3 & 0.7601 & 0.7599 & 0.7614 & \textbf{0.7618} \\
                        & 6 & 0.7601 & 0.7603 & 0.7597 & \textbf{0.7620} \\
                        & 9 & 0.7590 & 0.7602 & 0.7157 & \textbf{0.7624} \\
                        & 12 & 0.7575 & 0.7598 & 0.7170 & \textbf{0.7619} \\
   \bottomrule
\end{tabular}}
\end{table}
\begin{figure*}[t]
  \centering
  \subfigure[AUC/10Min of different models]{
  \includegraphics[width=0.45\textwidth]{figures/model-res.pdf}
  \label{fig:auc-models}
  }\hspace{-10pt}
  \subfigure[AUC/10Min of AdaMoE with different $\lambda$]{
  \includegraphics[width=0.45\textwidth]{figures/lambda-res.pdf}
  \label{fig:auc-lambda}
  }
%   \Description{Drift adaptation results.}
  \caption{AUC/10Min of (a) different models and (b)  $\lambda$.}
  \label{fig:auc-change-results}
\end{figure*}

\textbf{Evaluation Metrics}.
We adopt AUC as the evaluation metric.
In our setting, data is in the stream form and fed for training only once.
At each time step $t$, we use the first 80\% of data as training samples $\mathcal{D}_t^{train}$, and the rest 20\% as testing samples $\mathcal{D}_t^{test}$. The model is first trained with $\mathcal{D}_t^{train}$
then applied to $\mathcal{D}_t^{test}$.
The output pCTRs and the ground truth click labels of samples in $\mathcal{D}_t^{test}$ are stored to
% The above training-and-prediction process continues until the whole data stream is consumed.
% \hl{why a true 20\% holdout is necessary; why not report each prediction from before the weight update (i.e., progressive validation) @Yuejiang}
% We use the pCTRs and labels of all test samples to 
calculate the \textit{overall AUC}.
Furthermore, to better investigate the performance of models with stream data, we collect the stored pCTR and label of test samples every 10 minutes to calculate \textit{AUC/10Min}.

\subsection{Baseline and Settings}


We compare AdaMoE with the following baseline models.

$\bullet$ \textit{IncCTR}: 
% which has the same model structure as AdaMoE, but 
the pCTR is simply the average of all experts' output. 
% \hl{Shall we modify the name of IncCTR as mentioned by reviewer?@Yuejiang}

$\bullet$ \textit{MoE}: 
% which has the same model structure as AdaMoE, but 
the outputs of experts are aggregated by a gate network. The gate network used for the MoE baseline is a two-layer MLP with 64 and 32 neurons, respectively.

$\bullet$ \textit{IADM}: which stack ``experts'' in the depth direction, and the output of experts are also aggregated by a gate network. 
% Note that in IADM, the hidden units of MLP in each expert are set to [572, 572], so that the parameter numbers are the same as AdaMoE and other baselines.

For industrial dataset, we use DCN \cite{wang2017deep} and DIN \cite{zhou2018deep} as the backbone, respectively. For public dataset, we use DCN as backbone due to the absence of user behavior data in avazu dataset.
The output dimension of the backbone is 1024.
Each expert is a 2 layer MLP with [512, 256] hidden units and ReLU activation, combining a linear layer with the sigmoid function that maps to the predicted CTR.
The decayed factor is set to $\lambda=0.5$.
% All experiments were conducted on a machine with an NVIDIA 3090 GPU (24-GB memory), a 32-core AMD Ryzen Threadripper 3970X CPU (2.2GHz), and 250G of RAM.
% \subsection{Hyper-parameter Tuning}
We use the Adam optimizer for all methods. 
% In general, there are two hyper-parameters in training, including the learning rate and the batch size. 
% We try learning rate in \{$3\times10^{-2}$, $1\times10^{-2}$, $3\times10^{-3}$, $1\times10^{-3}$, $3\times10^{-4}$, $1\times10^{-4}$\} and batch size in \{1024,2048,4096\}. 
With grid search, the optimal learning rate is $1\times10^{-3}$ for AdaMoE and IADM, $1\times10^{-2}$ for IncCTR, and $3\times10^{-4}$ for MoE. 
% The optimal batch size is $4096$ for all models.
% \subsection{Baseline}
% \textbf{Baseline.} 




% \begin{itemize}
%   \item \textbf{IncCTR} which has the same model structure as AdaMoE, but the predicted CTR is simply the average of all experts output.
%   \item \textbf{MoE} which has the same model structure as AdaMoE, but the output of experts are aggregated by a gate network.
%   \item \textbf{IADM} which stack ``experts'' in depth direction, and the output of experts are also aggregated by a gate network. Note that in IADM, the hidden units of MLP in each expert is set to [572, 572], so that the parameter numbers are the same as AdaMoE and other baseline.
% \end{itemize}

% \textbf{Evaluation Metrics.} 


\subsection{Quantitative Results}
\textbf{Industrial Dataset}
% \textbf{Quantitative Results.} 
As shown in Table. \ref{tab:main-res}, AdaMoE outperforms all baseline models with \#exp. varying from three to twelve.
When the backbone is DIN and \#exp. is six, the overall AUC of AdaMoE improves by 0.19\% compared to the best baseline method (IADM with 3 experts).
The improvement of AUC is significant in CTR prediction \cite{wang2017deep,cheng2016wide,guo2017deepfm}.
% \textcolor{blue}{For AdaMoE, we can see that as the number of experts increases, the overall AUC is higher for both DCN and DIN backbone. This shows that more experts can improve the learning and representation ability of AdaMoE.
% However, for IADM, we can see that the too many experts can results in the decrease of overall AUC. This is because that  }
We obtain the best result when \#exp. is six for AdaMoE.
However, for IADM we can see that too many experts can result in performance degradation. 
since IADM ensembles experts vertically which can be problematic when depth of the network grows larger.
The case of the single expert (\#exp.=1) is plotted in Fig. \ref{fig:auc-models} since all methods degenerate to the same. All MoE based methods outperforms single expert network as expected.


\textbf{Public Dataset}. 
% We can observe the similar results over public dataset. That is, 
The proposed AdaMoE also performs better than other baseline methods at any \#exp.. 
% We do not consider the case where there is only one expert because all methods are identical at this time theoretically.
% Besides, we find that at any number of experts, AdaMoE performs the best. 
% This is because all baseline methods update models' parameters based on gradient descent. 
Since Avazu scales much smaller than industrial datasets, training based on gradient descent might be not efficient, especially for models with more parameters. While for AdaMoE, the update of expert weights is in closed-form and thereby more efficient. 
% Therefore, AdaMoE is trained more efficiently compared to other baseline models, and thus, yields better performance with more experts. 
Besides, we can see that AUC generally drops as \#exp. increases for baselines.
One possible reason is that due to the small scale of the public dataset, as \#exp. increases, the underfitting degree the model gradually increases. 


\subsection{Qualitative Results}

% \textbf{Qualitative Results.} 
To further study how the models handle the concept drift in streaming data, we plot the AUC/10Min in Fig. \ref{fig:auc-models}.
The \#exp. is set to six and the backbone model is DIN.
Similar results can be observed with other settings and are omitted here.
We marked 18:40 in Fig. \ref{fig:auc-models}, which corresponds to the occurrence of concept drift.
Before 18:40, the AUC/10Min of AdaMoE increases faster than other baselines, which means AdaMoE can quickly learn with stream data.
After 18:40, the AUC/10Min of all methods begins to drop.
Among all models, AdaMoE first stops the drop, and its decline is about 30\%-40\% less than other baselines, which means AdaMoE quickly adapts to new distribution and alleviates concept drift.
% We can see that AUC/10Min begins to increase at around 24:00.
% This further validates that AdaMoE is more robust and reliable.
% Also, the result of single expert (\#exp.=1) is plotted (purple line), and all MoE based methods outperforms single expert network as expected.
% \hl{Experiment: AdaMoE adapts to new distribution faster than MoE, and all methods are better than one-expert-model}

% \hl{Figure3, almost fixed gap between baselines and ours, expect to see baseline goes down dramatically, and ours recovered quickly. Also, complete one? or multiple days?}


\subsection{Influence of Decayed Factor $\lambda$.}
% \textbf{Influence of Decayed Factor $\lambda$.} 
% To further investigate the influence of decay rate $\lambda$, we show the AUC/10Min of AdaMoE with different $\lambda$ in Fig. \ref{fig:auc-lambda}.
We investigate the impact of the decayed factor $\lambda$ in Fig. \ref{fig:auc-lambda}.
When $\lambda$ is small, AdaMoE can quickly adapt to stream data, but
% and AUC/10Min increases before 18:00 and around 24:00.
% However, when  $\lambda$ is small, 
AUC/10Min fluctuates more and the model is unstable.
We empirically find $\lambda=0.5$ achieves a better tradeoff between the stability and adaptability of AdaMoE, and yields the best overall AUC. 


\subsection{Online A/B Testing}
The proposed AdaMoE model has been deployed in the online advertising system of one of the world's largest E-commerce companies.
The online A/B test lasts for a week (from 2022-Jan-7 to 2022-Jan-13).
Compared to the highly optimized base model, the proposed AdaMoE model contributes to 1.8\% CTR (Click Through rate) and 1.89\% eCPM (Effective Cost Per Mille) gain.

% \begin{figure}[!ht]
%  \centering
%   \includegraphics[width=0.8\textwidth]{figures/system-framework}
%   \caption{The architecture of the online model system}
%   \label{fig:system}
% \end{figure}

% \subsubsection{System Deployment}
% To conduct online A/B test, we deploy the proposed AdaMoE model in the online advertising system of one of the world's largest E-commerce companies.
% Fig. \ref{fig:system} depicts the architecture of the online advertising system.

% \textbf{Offline Batch Training}
% \textbf{Offline Inference and Training}



% \subsubsection{Online A/B testing}
% The online A/B test lasts for a week (from 2022-Jan-7 to 2022-Jan-13).
% Compared to the highly optimized base model, the proposed AdaMoE model contributes to 1.8\% CTR (Click Through rate) and 1.89\% eCPM (Effective Cost Per Mille) gain.

==> admoe_arxiv/methods.tex <==

\section{Methodology}


\subsection{Problem Definition}
In this work we consider CTR prediction with stream data.
Let $\{\mathcal{D}_t\}_{t=1}^{+\infty}$ be the stream data, where $\mathcal{D}_t = \left\{\mathbf{x}_{t, i}, y_{t, i}\right\}_{i=1}^{N_t}$ denotes the training data at time step $t$ and $(\mathbf{x}_{t, i}, y_{t, i})$ are generated i.i.d. from the density $P_t(X, y)$.
Here, $\mathbf{x}_{t, i}\in \mathbb{R}^f$ represents the data features of the $i$-th impressed advertisement at time step $t$, and
% It includes the advertisement' features, and the profile and behavioral features of the user to which the advertisement is exposed.
$y_{t, i} \in \{0, 1\}$ is the ground truth label indicating whether the user clicks the item.%impressed advertisement.
\subsection{Influence of Concept Drift}
% \hl{What is concept drift? What kind of concept drift we addressed here? And how it influence the CTR prediction?}\\
Concept drift problem refers to the phenomenon in which the statistical properties of data features and targets change in unforeseen ways over time\cite{lu2018learning}, and it happens at time step $t$ if $P_t(X, y)\neq P_{t+1}(X, y)$ \cite{ramirez2017survey}. 
% which may be caused by some hidden variables which cannot be measured directly . 
% \hl{how about periodical CD? whether we include time features? }
% Formally, concept drift is defined as follows:
% Assume the stream data in time step $t$ is $\mathcal{D}_t = \left\{\mathbf{x}_{t, i}, y_{t, i}\right\}_{i=1}^{N_t}$, where $(\mathbf{x}_{t, i}, y_{t, i})$ are generated i.i.d. from the probability density $P_t(X, y)$. 
% It happens at time step $t$ if $P_t(X, y)\neq P_{t+1}(X, y)$ \cite{ramirez2017survey}. 
% Since $P_t(X, y) = P_t(X)P_t(y|X)$, concept drift can be triggered by three sources: $P_t(X)$ drifts while $P_t(y|X)$ stays unchanged (virtual drift), $P_t(y | X)$ drifts while $P_t(X)$ stays unchanged (actual drift), and both $P_t(X)$ and $P_t(y|X)$ drift simultaneously (mix drift) \cite{ramirez2017survey}.
In the context of CTR prediction, the distribution of user-generated data steams consistently changed over time due to drifting user interests or user population.

\textbf{The influence of concept drift on model performance.} 
Suppose there is a predictor $F_t$ that predict the label for $\forall \mathbf{x}_t\sim P_t(\mathbf{x})$ perfectly, and the best predictor under some restrict class is $F_t^*$. However, under various restrictions, such as complexity, non-convexity and model selection, we can only find $\tilde{F}_t^*$ in real practice, which is an approximation of $F_t^*$. We can decompose the error of $\tilde{F}_t^*$ as

% Now we show that concept drift can influence the performance of the model, leading to poor predictions. 
% Let $\mathscr{F}$ be the unrestricted function class.
% For CTR prediction task at time $t$, the goal is to find a function $F_t \in \mathscr{F}$ s.t. $F_t(\mathbf{x}_t) = \arg\max_{y\in\{0, 1\}}P_t(y|\mathbf{x}_t)$ $\forall \mathbf{x}_t\sim P_t(\mathbf{x})$. However, $F_t$ is unavailable since its computation requires infinity sample size. With finite sample $\mathcal{D}_t = \left\{\mathbf{x}_{t, i}, y_{t, i}\right\}_{i=1}^{N_t}$ and restrict function class $\mathscr{F}^* \subset \mathscr{F}$, the optimal function is $F_t^* = \arg \min_{F \in \mathscr{F}^*}\sum_{i=1}^{N_t}l(F(\mathbf{x}_{t, i}), y_{t, i})\in \mathscr{F}^*$, where $l$ is any loss function, and $\mathscr{F}^*$ depends on the model class we choose. In real practice, under various restrictions, such as time and space complexity, convergence to sub-optimal issue due to non-convexity, and model selection etc., we can only find an approximation of $F_t^*$, i.e., $\tilde{F}_t^* \in \mathscr{F}^*$.

% With these definitions, the error of $\tilde{F}_t^*$ can be decomposed as
\begin{equation}
    \epsilon(\tilde{F}_t^*) - \epsilon(F_t) = \underbrace{\epsilon(\tilde{F}_t^*) - \epsilon(F_t^*)}_{\text{estimation error}} + \underbrace{\epsilon(F_t^*) - \epsilon(F_t)}_{\text{approximation error}} \label{eqn:error},
\end{equation}
where the estimation and approximation error reflects the inability of the learning algorithm and the lack of finite data, model selection and so on respectively. If concept drift occurs, the approximation error becomes $\epsilon(F_t^*) - \epsilon(F_{t+1})$, which is larger in most cases, thus the performance of the model is reduced. Therefore, when the metrics of the model such as AUC drops significantly, we should pay attention to whether there occurs concept drift.
% the data distribution changes from $P_t(X, y)$ to $P_{t+1}(X, y)$, and
% , while estimation error remains unchanged

\textbf{Why MoE structure can alleviate concept drift? }
% Concept drift influences the performance of the model by increasing approximation error in eqn. (\ref{eqn:error}), since 
The vanilla incremental learning methods (single estimator, i.e., one-expert-model) lacks robustness to changes over time. The basic idea is to construct $m$ experts to enhance robustness and accelerate adaptation to the new distribution.
The following inequality holds\cite{zeevi1998moe}:

\begin{equation}
    ||F-F^{(m)*}||_p\leq cm^{-\frac{r}{d}}, 1 \leq p < \infty,
\end{equation}
where $d$ is the input dimension, $F$ is a Sobolev class function of order $r$ in $L_p$ norm and $F^{(m)*}$ is the MoE function of $m$ experts. This inequality gives an upper bound of the approximation error, indicates the convergence of MoE, and
% . Besides, for any $F$ and $F^{(m)*}$ that satisfy the above assumption, the inequality 
gives an approximation that $F^{(m)*}$ can uniformly approximate $F$ at a rate of at least $\mathcal{O}(cm^{-\frac{r}{d}})$. Thus, if $F_t$ changes to $F_{t+1}$, the MoE model $F^{(m)*}_t$ can adapt to the new distribution  therefore alleviate concept drift.
% at a faster rate than the one-expert-model $F^*_t$,
%\hl{Motivation:why moe can alleviate CD?}

% \hl{Generality: Can adamoe be extended to multi-class classification or even regression??}

% \hl{The switch from "Why MoE can alleviate concept drift?" to "AdaMoE Framework" a bit abrupt? Say that our AdaMoE is based on MoE?}
% \begin{figure*}
%   \centering
%   \subfigure[6-hour vs. 6-hour similarity]{
%   \includegraphics[width=0.35\textwidth]{figures/similarity-new.pdf}
%   }
%   \subfigure[Variation of CTR]{
%   \includegraphics[width=0.32\textwidth]{figures/ctr-var.pdf}
%   }
% %   \Description{Empirical observation.}
%   \caption{Empirical observation of concept drift. (a) Impressed items are grouped every six hours, and the inter-group energy distance \cite{sugiyama2015introduction} is calculated and normalized.
%   Larger value denotes larger dissimilarity.
% %   The lower unified distance value is, the more similar two groups of samples are. 
%   (b) Real CTR within a day is shown in relative scale.}
%   \label{fig:drift}
% \end{figure*}
\subsection{Framework}
% In this paper, we propose the adaptive mixture of experts model (AdaMoE) to handle the concept drift in CTR prediction with stream data.
% \hl{@Fei how to connect cd and adamoe?}


%In this case, the approximation error can be represented as the combination of $\epsilon(F_t^{*(1)},F_t),...,\epsilon(F_t^{*(m)},F_t)$. If we combine these experts in an appropriate way, i.e., compute the aggregation weights which can minimize the loss of the model as much as possible, concept drift will be alleviated.\\
In this work, we propose the adaptive mixture of experts model (AdaMoE) in CTR prediction with stream data. As illustrated in Fig. \ref{fig:module}, the proposed AdaMoE consists of two modules: the \textit{main module} that uses the input data feature to predict the CTR, and the \textit{weights update module} that dynamically computes and updates the aggregation weights of all experts' predictions.

% In this work, we use ensemble methods to learn with data stream.
\subsubsection{Main Module}
In the main module, the representation $\mathbf{e}_{t, i}$ of sample $\mathbf{x}_{t, i}$ is first extracted with a backbone model, which can be DCN \cite{wang2017deep} or DIN \cite{zhou2018deep}, etc., and fed into $m$ experts.
% \begin{equation}
%   \mathbf{e}_{t, i} = Backbone(\mathbf{x}_{t, i}).
% \end{equation}
% The backbone model can be deep cross network (DCN) \cite{wang2017deep} or deep interest network (DIN) \cite{zhou2018deep}, etc., which depends on the used features.
% Then, the extracted representation $\mathbf{e}_{t, i}$ is fed into $m$ experts.
Each expert is an MLP network with a sigmoid activation.
All experts convert $\mathbf{e}_{t, i}$ to their own predicted CTR (pCTR) $\hat{y}_{t, i}^{(k)}$.
% where $\hat{\mathbf{y}}_{t, i} = [\hat{y}_{t, i}^{(1)}, \cdots \hat{y}_{t, i}^{(m)}]^T$ is the concatenation of the experts' pCTR.
% \begin{equation}
%   \hat{y}_{t, i}^{(k)} = Expert^{(k)}(\mathbf{e}_{t, i}).
% \end{equation}
Assume that all samples use the same aggregation weights, $\mathbf{w}_t = [w^{(1)}_{t}, \cdots, w^{(m)}_{t}]^T \in [0,1]^{m}$, to aggregate the output of experts, $||\mathbf{w}||_1=1$. Denote $\hat{\mathbf{y}}_{t, i} = [\hat{y}_{t, i}^{(1)}, \cdots \hat{y}_{t, i}^{(m)}]^T$, the pCTR is given by
\begin{equation}
  \hat{y}_{t, i} = \hat{\mathbf{y}}_{t, i} \cdot \mathbf{w}_{t} = \sum_{k=1}^{m} w^{(k)}_{t} \hat{y}_{t, i}^{(k)}.\label{eqn:pctr}
\end{equation}

In AdaMoE, we separate the training of the main module and the compute of experts' aggregation weights.
To train the main module, for the sample $\mathbf{x}_{t, i}$, we calculate the cross entropy loss
\begin{equation}
  \mathcal{L}_{CE}(t, i) = -(y_{t, i} \cdot \log(\hat{y}_{t, i}) + (1 - y_{t, i}) \cdot \log(1 - \hat{y}_{t, i})).\label{eqn:celoss}
\end{equation}
% Then, the total training loss for the main module at time $t$ is
% \begin{equation}
%   \mathcal{L}_{main}(t) = \sum_{i=1}^{N_t} \mathcal{L}_{CE} (t, i).\label{eqn:allloss}
% \end{equation}
The main module is optimized with gradient descent, but the data at time $t$ is used only once as the data is in stream form.

% \begin{figure}
%  \centering
%   \includegraphics[width=0.45\textwidth]{figures/AdaMoE}
%   \caption{An overview of AdaMoE.}
% %   \Description{AdaMoE Module.}
%   \label{fig:module}
% \end{figure}

\subsubsection{Weights Update Module}
\label{sec:weight-update}
\begin{algorithm}[t]
\SetAlgoLined
% \footnotesize
\KwIn{Data $\mathcal{D}_t = [\mathbf{x}_t, \mathbf{y}_t] = \left\{\mathbf{x}_{t, i}, y_{t, i}\right\}_{i=1}^{N_t}$.}
\KwOut{Predicted CTR $\hat{y}_{t, i}$ for each impressed advertisement.}
% \KwResult{Write here the result }

  {\nonl\footnotesize\texttt{// Forward: predict CTR}}\;

  $\hat{\mathbf{y}}_{t, i} \leftarrow \text{MainModule}(\mathbf{x}_{t, i})$; \hspace{3em}{\footnotesize\texttt{// Collect pCTR of experts}}\;

  $\hat{y}_{t, i} \leftarrow \hat{\mathbf{y}}_{t, i} \cdot \text{stopgrad}(\mathbf{w}_{t-1})$;\hspace{3em}{\footnotesize\texttt{// Aggregate pCTR of experts}}\;

  {\nonl\footnotesize\texttt{// Backward: update main module and aggregation weights}}\;

  $\tilde{\mathbf{y}}_{t, i} \leftarrow y_{t, i}\cdot \hat{\mathbf{y}}_{t, i} + (1-y_{t, i})\cdot (1-\hat{\mathbf{y}}_{t, i})$; 
  
  $\mathbf{w} \leftarrow \frac{1}{N_t}\sum_{i=1}^{N_t}\frac{\tilde{\mathbf{y}}_{t, i}}{||\tilde{\mathbf{y}}_{t, i}||_1}$; \hspace{3em}{\footnotesize\texttt{// Compute aggregation weights}}\;

  $\mathbf{w}_{t} \leftarrow \lambda\mathbf{w_{t - 1}} + (1-\lambda)\mathbf{w}$; \hspace{3em}{\footnotesize\texttt{// Update aggregation weights}}\;

  \caption{AdaMoE for CTR Prediction.}
\end{algorithm}

In this work, we aim to efficiently compute and update the aggregation weights of experts' predictions.
To achieve this, the aggregation weights should minimize the loss function and are easily computed.
%  so that AdaMoE can adapt to the concept drift in streaming data
% In the application of online CTR inference, we design an effective method to approximate the optimal aggregation weights of the experts.
We consider the computation of the aggregation weight at time step $t$ and omit script $t$ for simplicity. Based on Eqn. (\ref{eqn:pctr})(\ref{eqn:celoss}), the total loss to minimize at time $t$ is
% Let $y_i \in \{0, 1\}$ be the ground truth label of the $i$-th impressed advertisement and $\hat{y}_i^{(k)} \in [0, 1]$ be the predict CTR given by the $k$-th expert of the $i$-th impressed advertisement. 


\begin{equation}
    \mathcal{L} = -\sum_{i=1}^{N}(y_i\cdot\log\sum_{k=1}^{m} w^{(k)} \hat{y}_{i}^{(k)} + (1-y_i)\cdot\log\sum_{k=1}^{m} w^{(k)} (1-\hat{y}_{i}^{(k)})).\label{eqn:loss}
\end{equation}
Let $\tilde{y}_i^{(k)} = y_i\cdot \hat{y}_{i}^{(k)} + (1-y_i)\cdot (1-\hat{y}_{i}^{(k)})$, $\tilde{\mathbf{y}}_{i} = [\tilde{y}_{i}^{(1)}, \cdots \tilde{y}_{i}^{(m)}]^T$, 
\begin{equation}
    \mathcal{L} = -\sum_{i=1}^{N}(\log\sum_{k=1}^{m} w^{(k)} \tilde{y}_{i}^{(k)}) = -\sum_{i=1}^{N}(\log(\tilde{\mathbf{y}}_{i} \cdot \mathbf{w})).\label{eqn:loss_all}
\end{equation}
% \begin{small}
% \begin{align}
%   &\mathcal{L} = \sum_{i=1}^{N} \mathcal{L}_{CE} (i) \nonumber\\
%   &=-\sum_{i=1}^{N}(y_i\cdot\log\sum_{k=1}^{m} w^{(k)} \hat{y}_{i}^{(k)} + (1-y_i)\cdot\log(1-\sum_{k=1}^{m} w^{(k)} \hat{y}_{i}^{(k)}))\nonumber\\
%   &=-\sum_{i=1}^{N}(y_i\cdot\log\sum_{k=1}^{m} w^{(k)} \hat{y}_{i}^{(k)} + (1-y_i)\cdot\log\sum_{k=1}^{m} w^{(k)} (1-\hat{y}_{i}^{(k)}))\label{eqn:loss}
% \end{align}
% \end{small}
% \begin{align}
%   &\mathcal{L} = \sum_{i=1}^{N} \mathcal{L}_{CE} (i) \nonumber\\
%   &=-\sum_{i=1}^{N}y_i\cdot\log\sum_{k=1}^{m} w^{(k)} \hat{y}_{i}^{(k)}\nonumber\\
%   &-\sum_{i=1}^{N} (1-y_i)\cdot\log(1-\sum_{k=1}^{m} w^{(k)} \hat{y}_{i}^{(k)})\nonumber\\
%   &=-\sum_{i=1}^{N}y_i\cdot\log\sum_{k=1}^{m} w^{(k)} \hat{y}_{i}^{(k)}\nonumber\\
%   &-\sum_{i=1}^{N}(1-y_i)\cdot\log\sum_{k=1}^{m} w^{(k)} (1-\hat{y}_{i}^{(k)})\label{eqn:loss}
% \end{align}
The target is to minimize $\mathcal{L}$.
% \begin{equation}
%   \mathbf{w} = {\arg\min}_{||\mathbf{w}||_1=1} \mathcal{L}.\label{eqn:weight}
% \end{equation}
For simplicity, we ignore the partial derivative $\frac{\partial w^{(j)}}{\partial w^{(i)}}$ for $\forall i \neq j $. In fact, $\frac{\partial w^{(j)}}{\partial w^{(i)}}$ tends to $0$ as \#exp. increases. Then, $\mathcal{L}' := \frac{\partial \mathcal{L}}{\partial w} = -\sum_{i=1}^{N}\frac{\tilde{\mathbf{y}}_{i}}{\tilde{\mathbf{y}}_{i} \cdot \mathbf{w}} \leq 0$ since $\tilde{\mathbf{y}}_{i}$ and $\mathbf{w}$ are not less than $0$. Thus, we try to find $\mathbf{w}$ that can make $\mathcal{L}'$ closest to $0$ and maximize $\mathcal{L}'$ as much as possible.
% denote the partial derivatives of $\mathcal{L}$ with respect to $\mathbf{w}$ under this assumption as $\mathcal{L}'$.
% under the restriction $\sum_{k=1}^{m} w^{(k)}=1$ and $0\leq w^{(k)} \leq 1$ for $\forall k = 1,...,m$, i.e., $\mathbf{w} = \arg\max_{\mathbf{w}} \mathcal{L}'$.
% \begin{equation}
%   \mathbf{w} = \arg\max_{\mathbf{w}} \mathcal{L}'.
% \end{equation}
Noticed that $||\mathbf{w}||_2 \leq ||\mathbf{w}||_1 =1$ by Cauchy-Schwarz inequality, we can write $\mathcal{L}'$ as 
\begin{equation}
  \mathcal{L}' = -\sum_{i=1}^{N}\frac{\tilde{\mathbf{y}}_{i}}{||\tilde{\mathbf{y}}_{i}||_2||\mathbf{w}||_2\cos{\theta_i}} \leq -\sum_{i=1}^{N}\frac{\tilde{\mathbf{y}}_{i}}{||\tilde{\mathbf{y}}_{i}||_2}\cdot\frac{1}{\cos{\theta_i}}, \label{eqn:simple}
\end{equation}
where $\theta_i$ is the angle between $\tilde{\mathbf{y}}_{i}$ and $\mathbf{w}$.
% , and  $||\cdot||_2$ means $2$-norm. 
% It is difficult to find $\mathbf{w} = \arg\max_{\mathbf{w}} \mathcal{L}'$ directly. \\
% Noticed that $||\mathbf{w}||_2 \leq ||\mathbf{w}||_1 =1$ by Cauchy-Schwarz inequality. Then,
% , where $||\cdot||_1$ means $1$-norm. In fact, it is easy to prove that $||\mathbf{w}||_2 \leq ||\mathbf{w}||_1 \leq \sqrt{m}||\mathbf{w}||_2$ by simply applying Cauchy-Schwarz inequality. Then, 
% \begin{equation}
%     \mathcal{L}' \leq -\sum_{i=1}^{N}\frac{\tilde{\mathbf{y}}_{i}}{||\tilde{\mathbf{y}}_{i}||_2}\cdot\frac{1}{\cos{\theta_i}}. \label{eqn:simple}
% \end{equation}
Instead of directly finding $\mathbf{w}$ that maximize $\mathcal{L}'$, we maximize the right hand side of eqn.  (\ref{eqn:simple}). For $i$-th impressed advertisement, $\frac{1}{\cos{\theta_i}}$ reachs its minimum when $\cos{\theta_i} = 1$, i.e., $\tilde{\mathbf{y}}_{i}$ and $\mathbf{w}$ are collinear and $\mathbf{w} = \frac{\tilde{\mathbf{y}}_{i}}{||\tilde{\mathbf{y}}_{i}||_1}$. To be fair to each impressed advertisement, let 

\begin{equation}
    \mathbf{w} = \frac{1}{N}\sum_{i=1}^{N}\frac{\tilde{\mathbf{y}}_{i}}{||\tilde{\mathbf{y}}_{i}||_1}, \label{eqn:w}
\end{equation}
$\mathbf{w}$ is initialized as $\mathbf{w}_0=[\frac{1}{m}, \frac{1}{m},...,\frac{1}{m}]^T \in \mathbb{R}^{m}$. Monte Carlo simulation is conducted to examine approximation capability. $\mathcal{L}$ computed with eqn. \ref{eqn:w} is approximately equals to the minimum of $\mathcal{L}$ at 90\% significance level. 

% \begin{table}[t]
%   \caption{Loss of different $\mathbf{w}$ in Monte Carlo experiment} 
%   \label{tab:loss}
%   \centering
% %   \small
% \begin{tabular}{c|c|ccc}
%    \toprule
%     & \#(Experts) & min$\mathcal{L}$ & max$\mathcal{L}$ & our$\mathcal{L}$ \\
%    \midrule
%    \multirow{4}{*}{loss} & 3 & 0.7539 & 1.0347 & 0.7567 \\
%                         & 6 & 0.7209 & 0.8924 & 0.7247 \\
%                         & 9 & 0.7095 & 0.7702 & 0.7107 \\
%                         & 12 & 0.7052 & 0.7450 & 0.7082 \\
%    \bottomrule
% \end{tabular}
% \end{table}
% \textbf{Monte Carlo experiment.} 
% To further illustrate the approximation capability of eqn. (\ref{eqn:w}), we perform a Monte Carlo experiment. Assume the sample size is $1024$, and the number of experts is $6$, that is,  $N = 1024$, $m = 6$. Since the predict CTRs are all in $[0, 1]$, we sample $\hat{y}_{i}^{(k)} \sim i.i.d. U(0, 1)$ and $y_i \sim i.i.d. Binom(1, 0.5)$. Then, we fix all $\hat{y}_{i}^{(k)}$ and $y_i$, and sample $\mathbf{w} \in [0, 1]^m$ for $1000000$ times, compute the loss function with eqn. (\ref{eqn:loss}), then find the minimum value and the maximum value, which is almost the true minimum and maximum of $\mathcal{L}$. We also compute $\mathcal{L}$ with eqn. (\ref{eqn:w}). As shown in Table. \ref{tab:loss}, which shows the result of one Monte Carlo experiment when $m = 3, 6, 9, 12$, the loss computed with eqn. (\ref{eqn:w}) is very close to the minimum. Besides, the loss computed with eqn. (\ref{eqn:w}) is less than about $95\%$ of all $1000000$ losses in most of the Monte Carlo experiments.



\textbf{Weight Update Rule. }\label{sec:weight-update}
The aggregation weight (eqn. (\ref{eqn:w})) considers only the information in time step $t$. Considering historical information, we introduce a decay factor $\lambda$ into the update rule of aggregation weight, and the aggregation weights at time step $t$ is 
\begin{equation}
    \mathbf{w_t} = \lambda\mathbf{w_{t - 1}} + (1 - \lambda)\mathbf{w},\text{where }\mathbf{w} = \frac{1}{N_t}\sum_{i=1}^{N_t}\frac{\tilde{\mathbf{y}}_{t, i}}{||\tilde{\mathbf{y}}_{t, i}||_1},
\end{equation}
where decayed factor $\lambda \in [0, 1)$. $\lambda = 1$ is not considered because we ignore the case where $w$ is not updated with current information.
To sum up, 
% we can use the ground truth and predicted CTR to compute and update the aggregation weights at each time step efficiently. 
we summarize the process of AdaMoE in Algorithm 1. Besides, the proposed approach is easy to be generalized to multi-class setting through the similar way of defining $\mathcal{L}_{CE}(i)$ and $\tilde{y}_{i}^{(k)}$.

\textbf{Why AdaMoE works?} The $k$-th expert works well at time step $t$ when its prediction $\hat{y}_{t, i}^{(k)}$ is close to the ground truth $y_{t, i}$, i.e. $\tilde{y}_{t, i}^{(k)}$ is close to $1$. AdaMoE analytically gives the aggregation weights that minimize the loss function, and gives larger weights to those experts that work better
% , gives smaller weights to those experts that work worse
. Thus, AdaMoE can find the better-performing expert from $m$ experts and give larger weights fast and precisely. Besides, AdaMoE also considers the history information, which contains the performance of each expert at historical time steps.

%\hl{Why AdaMoE works better than MoE?}

% \hl{Theoretical proof: The parameter update speed of AdaMoE is faster than that of MoE}

% \textbf{Generality Analysis.}
% The proposed approach can be easily generalized to multi-class setting. Omitting script $t$ for simplicity, for the sample $\mathbf{x}_{i}$, the cross entropy loss is $\mathcal{L}_{CE}(i) = -\sum_{l=1}^cy_{i, l} \cdot \log(\hat{y}_{i, l})$, where $c$ is the number of classes and $y_{i, l} \in \{0,1\}$, $\hat{y}_{i, l}\in [0,1]^m$  are the target and prediction for the sample $\mathbf{x}_{i}$ and class $l$, respectively. For the sample $\mathbf{x}_{i}$ in class $l_i$, $y_{i, l_i}=1$, and let $\tilde{y}_i^{(k)}=\hat{y}_{i, l_i}^{(k)}$ be the $k$-th expert's prediction of the probability that sample $\mathbf{x}_{i}$ belongs to class $l_i$, $\tilde{\mathbf{y}}_{i} = [\tilde{y}_{i}^{(1)}, \cdots \tilde{y}_{i}^{(m)}]^T$. Thus, the total loss is $\mathcal{L} = \sum_{i=1}^{N} \mathcal{L}_{CE} (i) = -\sum_{i=1}^{N}\log(\hat{y}_{i, l_i}) = -\sum_{i=1}^{N}\log(\sum_{k=1}^{m} w^{(k)} \tilde{y}_{i}^{(k)})=-\sum_{i=1}^{N}(\log(\tilde{\mathbf{y}}_{i} \cdot \mathbf{w}))$, which is the same as eqn. (\ref{eqn:loss_all}), and the way to find the aggregation weight is also the same.

% \subsection{Baseline - Mixture of Experts}
% To aggregate the prediction of each experts, mixture of experts (MoE) model \cite{ShazeerMMDLHD17} uses a gate network to map the representation $\mathbf{e}_{t, i}$ to the aggregation weights $\mathbf{w}_{t, i} = [w^{(1)}_{t, i}, \cdots, w^{(m)}_{t, i}]^T \in [0,1]^m$, that is,
% \begin{equation}
%   \mathbf{w}_{t, i} = Gate(\mathbf{e}_{t, i}).
% \end{equation}
% In the gate network, the $softmax$ function is applied to ensure that the output aggregation weights are all positive and sum to 1.
% Consequently, the final predicted CTR is given by
% \begin{equation}
%   \hat{y}_{t, i} = \mathbf{w}_{t, i}^T \hat{\mathbf{y}}_{t, i} = \sum_{k=1}^{m} w^{(k)}_{t, i} \hat{y}_{t, i}^{(k)}
% \end{equation}

% Although the MoE model is widely adopted in different fields and yields significant performance, training MoE can be challenging.
% For example, to mitigate the ``dead gate'' issue \cite{ShazeerMMDLHD17}, an auxiliary loss with a carefully tuned hyper-parameter is often required.
% This requires all training data are available and using (mini) batch gradient descent algorithm to train.
% However, in our scenario where data is in stream form, and cannot be cached in memory.
% Furthermore, it is often require model to converge fast to achieve better performance in online training \cite{YangZZX019}.
% Thus, it is not suitable to directly apply mature training techniques for MoE model with stream data.

% \subsection{Adaptive Mixture of Experts}

% \subsubsection{Main Module}
% The main module of AdaMoE is similar to the MoE model, that is, there is a backend which transform input features $\mathbf{x}_{t,i}$ into embedding $\mathbf{e}_{t, i}$, and $m$ experts network which consume the embedding $\mathbf{e}_{t, i}$ and output the predicted CTR $\hat{y}_{t, i}^{(k)}$.
% Different from the MoE model, in the main module of AdaMoE, we independently train each expert.


% \subsection{Adaptive Filter Theory in a Nutshell}
% We first briefly introduce adaptive filter theory \cite{haykin2008adaptive}. In the adaptive filter theory, there are $m$ sensors collecting data at each snapshot to recover 
